Isogeometric Analysis of the Gray-Scott Reaction-Diffusion Equations for Pattern Formation on Evolving Surfaces and Applications to Human Gyrification

We propose a numerical scheme based on the principles of Isogeometric Analysis (IgA) for a geometrical pattern formation induced evolution of manifolds. The development is modelled by the use of the Gray-Scott equations for pattern formation in combination with an equation for the displacement of the manifold. The method forms an alternative to the classical finite-element method. Our method is based on partitioning the initially spherical geometry into six patches, which are mapped onto the six faces of a cube. Major advantages of the new formalism are the reconstruction of the manifold based on bicubic spline-functions used for the computation of the concentrations as well as the evolution of the mapping operator. These features give a smooth representation of the manifold which, in turn, may lead to more realistic results. The method successfully reproduces the smooth but complicated geometrical patterns found on the surface of human brains.

==> preface.tex <==
\chapter*{Preface}
\setheader{Preface}

Before you lies the thesis "Isogeometric Analysis of a Reaction-Diffusion Model for Human Brain
Development" which has been written to fulfill the graduation requirements of the Applied Mathematics Program at the Delft University of Technology. I was engaged in this project from March 2015 to January 2016. \\
I chose for a subject related to the finite element method (FEM) since I had already been confronted with topics from numerical linear algebra during my project "The Scattering Algorithm for Sparse Linear Hermitian Systems", which would have been my first choice otherwise.  \\
This thesis is written for people with a background in (applied) mathematics and numerical analysis in particular. I have done my best to translate the basic principles of differential geometry into a formalism that is compatible with the formalism that is common in FEM-related topics. \\
I would like to thank my thesis supervisors Dr. ir. F.J. Vermolen and Dr. M. M\"oller for providing me with this exciting and challenging project and for their support and plenty of helpful advice during my time at the department. Furthermore, I would like to thank Joost for his help with the implementation of the numerical solver and for helping me improve my mathematical, as well as my programming skills with his useful tips.  \\
I would like to thank my parents for encouraging me to pursue a double degree despite the additional study costs associated with it. \\
Last but not least, I would like to thank everyone who takes his time to read this (rather lengthy) thesis.


\begin{flushright}
{\makeatletter\itshape
    \@author \\
    Delft, January 2016
\makeatother}
\end{flushright}



==> title.tex <==
\begin{titlepage}


\begin{center}

%% Insert the TU Delft logo at the bottom of the page.

%% Print the title in cyan.
{\makeatletter
\largetitlestyle\fontsize{64}{94}\selectfont\@title
%\largetitlestyle\color{tudelft-cyan}\Huge\@title
\makeatother}

%% Print the optional subtitle in black.
{\makeatletter
\ifx\@subtitle\undefined\else
    \bigskip
   {\tudsffamily\fontsize{22}{32}\selectfont\@subtitle}    
    %\titlefont\titleshape\LARGE\@subtitle
\fi
\makeatother}

\bigskip
\bigskip

by
%door

\bigskip
\bigskip

%% Print the name of the author.
{\makeatletter
%\largetitlefont\Large\bfseries\@author
\largetitlestyle\fontsize{26}{26}\selectfont\@author
\makeatother}

\bigskip
\bigskip

to obtain the degree of Master of Science
%ter verkrijging van de graad van Master of Science

at the Delft University of Technology,
%aan de Technische Universiteit Delft,

to be defended publicly on Tuesday January 28, 2016 at 02:00 PM.
%in het openbaar de verdedigen op dinsdag 1 januari om 10:00 uur.

\vfill

\begin{tabular}{lll}
    Student number: & 1545337 \\
    Project duration: & \multicolumn{2}{l}{March 18, 2015 -- January 28, 2016} \\
    Thesis committee: & Dr.\ ir.\ F.\ J.\ Vermolen, & TU Delft, supervisor \\
				   & Dr.\ M.\ M\"oller, & TU Delft, supervisor \\
        & Prof.\ dr.\ ir. \ C.\ Vuik, & TU Delft \\
        & Dr.\ ir.\ W.\ T. \ van Horssen, & TU Delft
\end{tabular}
%% Only include the following lines if confidentiality is applicable.

\bigskip
\bigskip
\emph{This thesis is confidential and cannot be made public until January 28, 2016.}
%\emph{Op dit verslag is geheimhouding van toepassing tot en met 31 december 2013.}

\bigskip
\bigskip
An electronic version of this thesis is available at \url{http://repository.tudelft.nl/}.
%\\[1cm]

%\centering{\includegraphics{cover/logo_black}}


\end{center}

\begin{tikzpicture}[remember picture, overlay]
    \node at (current page.south)[anchor=south,inner sep=0pt]{
        \includegraphics{cover/logo_black}
    };
\end{tikzpicture}

\end{titlepage}


